Agentic Relative Camera Pose Estimation via Learned Ranking and Verification

A wide range of approaches have been developed for camera pose estimation, including correspondence-based methods, end-to-end pose regression, and recent 3D geometric foundation models. Our key observation is that no single estimator is optimal for diverse challenges, such as wide baselines, lack of texture, appearance changes, and occlusions. Further analysis reveals substantial performance variation across both benchmarks and individual image pairs, with different estimators exhibiting complementary strengths. We introduce PoseAgent, an agentic framework for relative camera pose estimation that dynamically orchestrates pose estimators through learnable ranking and verification. Given an image pair, a profiling agent first extracts appearance, semantic, and geometric features relevant to pose estimation, e.g., scene type. A learned ranking agent then predicts the relative competence of multiple pose estimators given the image-pair profile. The top-ranked estimator is executed, and its predicted pose is assessed by a learned verification agent that estimates the corresponding pose error. When verification fails, PoseAgent adaptively invokes lower-ranked estimators until a candidate is accepted or the execution budget is reached. For pose verification, our verification network predicts pose errors more accurately than prior models. For pose estimation, PoseAgent improves AUC@5 degree up to 4.2% over the strongest standalone estimator on each of ARKitScenes, MegaDepth, ScanNet++, and RealEstate10K. On ARKitScenes, PoseAgent also outperforms VLM-based agents, which include a VLM ranker with the same verifier and fallback policy. These results demonstrate the effectiveness of our learned ranking and verification.

==> sections/2introduction_backup.tex <==
\section{Introduction}

Camera pose estimation is an important problem in computer vision and serves as a key component in applications such as virtual and augmented reality, autonomous navigation, 3D/4D reconstruction, and robotics.
%
Relative camera pose estimation aims to recover the 6 degree-of-freedom (6-DoF) transformation between camera coordinate systems of two images, with many approaches developed including sparse keypoint-based methods~\cite{lowe2004distinctive,nister2004efficient,detone2018superpoint,sarlin2020superglue}, dense correspondence-based methods~\cite{sun2021loftr,edstedt2024roma}, direct pose regression~\cite{kendall2015posenet,dong2025reloc3r}, and recent geometric foundation models~\cite{dust3r_cvpr24,mast3r_eccv24,wang2025vggt}.
%
A classical pipeline consists of feature detection, description, and matching.
%
These components have been modernized with learning-based methods, including deep keypoint detection~\citep{yi2016lift,detone2018superpoint,dusmanu2019d2,tyszkiewicz2020disk}, description~\citep{mishchuk2017working,tian2019sosnet}, matching~\citep{sarlin2020superglue,lindenberger2023lightglue,sun2021loftr}, and eventually end-to-end pose estimation~\cite{dong2025reloc3r,wang2025vggt}.

%More recent approaches further move toward dense correspondence estimation, such as RoMa~\citep{edstedt2024roma}, or directly regress the relative camera pose in an end-to-end manner~\citep{arnold2022map,ding2019camnet,khatib2024leveraging,zhou2020learn,winkelbauer2021learning,dong2025reloc3r}.

Despite substantial progress with a zoo of models developed, relative pose estimation is not a solved problem, in particular for challenges such as large viewpoint changes, wide baselines, textureless regions, repetitive structures, and scene dynamics.
%
We systematically evaluated many models and observed that no single pose estimator consistently performs the best for all datasets.
%
Interestingly, even classical or seemingly outdated estimators outperform more recent models in many cases, see detailed analysis in Section~\ref{sec:best_model_analysis}.
%

Our observations suggest that relying on a single universal pose estimator can be restrictive.
% the long-standing goal of developing a single universal pose estimator is unnecessarily restrictive.
%
Different pose estimators exhibit distinct strengths and weaknesses under different challenges.
%
For example, structure-based methods are highly accurate when reliable feature matches are available, but degrade under large viewpoint changes or limited visual overlap.
%
In contrast, end-to-end regression methods are more robust for these challenges, while being less accurate than structure-based methods when reliable geometric correspondences are available.
%
Rather than developing a single model, we ask which estimator is most suitable for a particular image pair, i.e., \textit{model selection}.
%
The need for model specialization is already reflected in existing systems. For example, SuperGlue~\cite{sarlin2020superglue} and RoMa~\cite{edstedt2024roma} provide separate models for indoor and outdoor scenes. However, such dataset-level specialization remains coarse. Image pairs can exhibit substantially different challenges, including limited overlap, wide baselines, textureless regions, repetitive structures, occlusions, and appearance changes.
%
This motivates selecting the most suitable estimator based on the characteristics of each individual image pair.
%
% What's more, 
Moreover, since the ground-truth camera pose is unavailable at inference time, the system must determine whether a predicted pose can be trusted.
%

%\emph{which pose estimator is globally the best}, we ask \emph{which estimator is most suitable for a particular image pair}.
%Answering this question at inference time is challenging because the ground-truth relative pose is unavailable. Moreover, selecting an estimator based only on its expected performance is insufficient, since even a highly ranked method can occasionally fail. An effective system should therefore not only predict which estimator is likely to succeed, but also evaluate the reliability of its output and adapt its decision when necessary.

Recent agentic vision systems~\cite{zuo20254kagent,lu2023chameleon} have shown that visual tasks can benefit from decomposing inference into profiling, planning, tool selection, execution, and feedback, rather than relying on a single model.
%
To leverage the complementary benefits of various pose estimators, we introduce \textbf{PoseAgent}, an agentic framework for relative camera pose estimation based on learnable ranking and verification.
%
PoseAgent treats multiple heterogeneous pose estimators as specialized tools and dynamically orchestrates them for each input image pair.
%
% The framework operates as a closed-loop inference process consisting of profiling, ranking, execution, and verification.
%
The framework operates as a closed-loop agentic inference process, in which profiling characterizes the image pair, ranking plans the order of tool calls, verification provides feedback on each tool output, and the ranking and verification decisions are learned directly from pose supervision.


Given an image pair, a profiling agent first extracts semantic and geometric characteristics using a collection of computer vision and image-processing tools.
%
These characteristics describe factors relevant to pose estimation, such as visual overlap, appearance variation, scene structure, and matching difficulty.
%
Based on the resulting profile, a learnable ranking agent predicts the relative competence of a set of candidate pose estimators.
%
The highest-ranked estimator is then executed to produce a candidate pose.
%
Importantly, estimator selection is not treated as a one-shot decision.
%
A learnable verification agent evaluates the reliability of the predicted pose using geometric evidence, without access to the ground-truth camera pose.
%
If the candidate fails verification, PoseAgent adaptively falls back to the next promising estimator according to the ranking.
%
In this way, ranking provides a prior estimate of estimator competence, while verification provides feedback about the reliability of the actual prediction, enabling closed-loop recovery from unsuccessful estimator choices.

%This formulation differs from conventional ensemble or model-selection approaches in several important ways. First, PoseAgentperforms \emph{instance-adaptive} estimator selection rather than choosing a globally optimal model. Second, the ranking and verification modules address complementary aspects of the problem: the former predicts which estimator is likely to succeed before execution, while the latter evaluates whether a produced pose should actually be trusted. Third, the verification signal enables adaptive test-time computation, allowing the framework to terminate early for easy image pairs while invoking additional estimators only when necessary. Thus, the proposed framework transforms relative camera pose estimation from a single-model prediction problem into an adaptive decision process over specialized geometric tools.

%We evaluate PoseAgenton multiple challenging relative pose estimation benchmarks, including MegaDepth1500, ARKitScenes1095, and ScanNet1500. Our experiments reveal substantial complementarity among existing pose estimators and show that the proposed ranking module can effectively predict their relative competence at the image-pair level. We further demonstrate that our learned verifier substantially improves the reliability of candidate-pose assessment and enables effective recovery from failed predictions. Combining these components, PoseAgentachieves state-of-the-art performance on MegaDepth1500 and ARKitScenes1095 and competitive performance on ScanNet1500. We additionally compare against general-purpose vision-language-model-based agents and find that specialized learnable ranking and verification provide more effective orchestration for relative camera pose estimation. These results suggest that agentic inference need not rely on a general-purpose language model; instead, task-specific competence estimation and verification can provide an effective mechanism for adaptive tool use in geometric computer vision.

Our main contributions are summarized as follows:
\begin{itemize}
\item Our analysis reveals substantial complementarity among existing pose estimators across datasets and individual image pairs, motivating instance-adaptive model selection rather than reliance on a single universal estimator.

%\item We develop a learnable ranking module given image profile for instance-adaptive model selection beyond the coarse specification of indoor/outdoor models.

\item We introduce {PoseAgent}, an agentic framework that integrates image-pair profiling, estimator ranking, execution, and verification into a closed-loop inference process, with learnable ranking and verification modules that respectively predict estimator competence for each image pair and assess the reliability of candidate pose estimates.

\item Extensive experiments demonstrate that {PoseAgent} outperforms standalone models for multiple datasets including ARKitScenes, MegaDepth, RealEstate10K, and ScanNet++, and outperforms VLM-based agents on ARKitScenes, including a VLM ranker that uses the same verifier and fallback policy.

% \item We introduce {PoseAgent}, an agentic framework for relative camera pose estimation that integrates image-pair profiling, estimator ranking, execution, and verification into a closed-loop inference process.
% \item We develop learnable ranking and verification modules that respectively predict estimator competence for each image pair and assess the reliability of candidate pose estimates, enabling adaptive model selection beyond indoor/outdoor and orchestration.

% \item Extensive experiments demonstrate that {PoseAgent} outperforms standalone models for multiple datasets including ARKitScenes, MegaDepth, RealEstate10K, and ScanNet++.
% %state-of-the-art performance on MegaDepth1500 and ARKitScenes1095 and competitive performance on ScanNet1500, while outperforming general-purpose VLM-based agent baselines for relative camera pose estimation.
% \item {PoseAgent} also outperforms general-purpose LLM/VLM agents equipped with pose-estimation tools, demonstrating the advantage of our learned ranking and verification.
\end{itemize}




==> sections/3related_work_backup.tex <==
\section{Related Work}
\label{related_work}

\paragraph{Relative Camera Pose Estimation.}
%Relative camera pose estimation has traditionally been addressed using correspondence-based geometric approaches. 
Conventional methods first detect and describe local features using hand-crafted operators, e.g., SIFT~\citep{lowe2004distinctive}
%FAST~\citep{rosten2006machine}, 
and SURF~\citep{bay2006surf}, then establish feature correspondences through descriptor matching, and recover the relative pose using multi-view geometric solvers~\citep{multiviewgeometry}.
With the advance of deep learning, the individual components have progressively been replaced by learned detectors, descriptors, and sprase/dense matchers. Examples of representative work include SuperPoint~\citep{detone2018superpoint}, SuperGlue~\citep{sarlin2020superglue}, LightGlue~\citep{lindenberger2023lightglue}, LoFTR~\citep{sun2021loftr}, and RoMa~\citep{edstedt2024roma}.
%improve correspondence estimation under challenging appearance and viewpoint changes. 
Furthermore, pose regression methods directly predict camera transformations given an image pair, bypasing explicit correspondence matching~\citep{kendall2015posenet,arnold2022map,ding2019camnet,khatib2024leveraging,zhou2020learn,winkelbauer2021learning,dong2025reloc3r}. 
More recently, large-scale 3D geometric foundation models, such as DUSt3R~\citep{wang2024dust3r}, Reloc3r~\citep{dong2025reloc3r}, and VGGT~\citep{wang2025vggt}, leverages Transformer architectures and diverse 3D training data to solve multiple geometric computer vision tasks including camera pose estimation.
%learn transferable geometric representations for camera pose estimation and other 3D perception tasks.
%
These developments have introduced a zoo of relative pose estimators with different architectures, assumptions, and failure modes, which motivates our method of model selection.

\paragraph{Model Selection and Pose Verification}
Adaptive selection among pose estimation strategies has been explored in several directions. 
Hybrid Camera Pose~\citep{camposeco2018hybrid} dynamically adjusts the sampling probabilities of different solvers within the estimation framework.
~\cite{yu2025relative} combines depth-aware and classic point-based solvers within a hybrid estimation pipeline and evaluates the resulting hypotheses using geometric constraints.
FAR~\citep{rockwell2024far} further points out the complementary strengths of geometric solvers and learned pose predictors, and learns to balance their predictions.
More recently, \cite{panek2026combining} adaptively select between structure-based and structure-less localization approaches by selecting pose estimate scoring function.
These studies demonstrate the value of adapting the estimation strategy to the input images. 
However, their selection strategies are typically performed at the solver level or between a small number of predefined estimation paradigms. 
In contrast, we formulate model selection as an explicit ranking problem over multiple standalone estimators, spanning correspondence-based methods, direct pose regression models, and large-scale 3D geometric models. \todo{add paper suggested by Carl}

Pose verification provides a complementary mechanism for assessing whether an estimated pose should be trusted. Traditional verification approaches rely on geometric consistency measures, such as epipolar verification, Sampson distance, reprojection error, and inlier-based RANSAC scores. These criteria provide interpretable geometic evidence, but their reliability can degrade when the supporting correspondences or geometric priors are sparse, as may occur under low overlap, textureless regions, large viewpoint changes, or substantial appearance variation. Learned verification offers an alternative by directly estimating the quality of a candidate pose hypotheses from visual and spatial evidence. For example, FSNet~\citep{barroso2023two} learns to score two-view geometric hypotheses from an image pair without depending on explicit correspondence-based features. Our verifier follows this learned-verification paradigm, but operates on final relative pose predictions produced by different estimators and is integrated with the estimator ranking stage. As a result, ranking and verification address two complementary questions: which estimator is most suitable for a given image pair, and whether the pose produced by that estimator should be accepted.% or replaced by an alternative. 

\textbf{Multimodal Large Language Model Agent}
Large language models have achieved increasingly capable  agents for planning, reasoning, and tool use~\citep{yao2022react, hong2023metagpt, wang2023describe, hu2025g2vlmgeometrygroundedvision, zuo20254kagent, szot2025multimodal, xu2026area3d, yao2026photoagent, zhang2026predicting}.
Early multimodal agents often relied on converting non-textual inputs, particularly images, into textual descriptions that could subsequently be processed by an LLM~\citep{wu2023visual,suris2023vipergpt, yang2023mm, gao2023assistgpt}. 
With the emergence of native multimodal models, visual perception and language-based instruction understanding can instead be integrated within a shared reasoning framework. 
Despite these advances, many vision tasks require specialized geometric or spatial information that is difficult to obtain through generic semantic perception alone~\citep{deng2026lostspacevisionlanguagemodels, ma2024spatialpin, guo2025pursuing, marsili2025visual}.
Multimodal agents therefore increasingly rely on external vision or geometry tools to acquire task-specific evidence during reasoning and planning~\citep{cho2026spatialclaw, guo2025pursuing, zuo20254kagent, wang2025vggt, leroy2024grounding, kirillov2023segment}. 
The resulting intermediate outputs can then be interpreted and aggregated by a reasoning module or through multi-agent collaboration, to support downstream decisions~\citep{guo2025pursuing, ma2024spatialpin, marsili2025visual}.
Our work follows this tool-augmented agentic paradigm and focuses on relative camera pose estimation. 
% Instead of relying on a single pose estimator, the agentic framework reasons over complementary pose estimators, ranks them according to characteristics of given image pairs, and verifies their outputs before producing the final relative pose. 


% While LLMs have achieved significant performance in powering text-based agents, multiple works also focus on extending these decision-making and reasoning abilities into the multimodal domain, by leveraging the more powerful Multimodal Large Language Models (MLLMs)~\citep{bai2025qwen2,dubey2024llama,Qwen3-Omni,zhu2025internvl3,team2025gemma,an2025llava,team2025qwen3,meta2025llama,comanici2025gemini}.
% In early works, the perception of multimodal agents relies on converting non-text inputs (usually images) into text descriptions ~\citep{wu2023visual,suris2023vipergpt,yang2023mm,gao2023assistgpt}, so that they are perceivable by LLMs.
% With the inherent multimodal ability in MLLMs, this perception process can be integrated with instruction understanding from users' inputs.
% While most MLLMs focus on the semantic understanding of non-textual inputs, many multimodal tasks require a more specialized perception, such as segmentation~\citep{ma2024spatialpin,zhang2024agent3d}, visual grounding~\citep{gou2024navigating,xu2024vlm,yang2024llm}, 3D reconstruction~\citep{ma2024spatialpin,guo2025pursuing,marsili2025visual}, etc.
% The requirements of such specialized information come from the planning process of the agent, which usually involves using specialized external tools~\citep{wang2025vggt,leroy2024grounding,kirillov2023segment}.
% After obtaining the specialized information required by the multimodal tasks, this intermediate information needs to be converted to text format and processed again by LLMs to generate final responses.
% This process often involves multi-agent collaboration, where a reasoning agent will be responsible for analyzing and aggregating intermediate information into a reasonable response ~\citep{guo2025pursuing,ma2024spatialpin,marsili2025visual}.


% \paragraph{Structure-based pose estimation}
% Structure-based methods estimate relative poses by detecting and matching keypoints from two images, followed by geometric pose estimation based on multi-view geometry~\citep{multiviewgeometry}.
% Traditional methods usually rely on hand-crafted and gradient-based features for keypoint detection and description, such as SIFT~\citep{lowe2004distinctive}, Harris corners~\citep{harris1988combined}, FAST~\citep{rosten2006machine}, and SURF~\citep{bay2006surf}. Correspondences are then established by nearest-neighbor search in the descriptor space and subsequently used to recover the relative camera pose through geometric solvers.
% With the advent of deep learning, individual components of this paradigm, including keypoint detection, feature description, and feature matching, have increasingly been replaced by neural networks. Learning-based detectors~\citep{yi2016lift,detone2018superpoint,dusmanu2019d2,tyszkiewicz2020disk} and descriptors~\citep{mishchuk2017working,tian2019sosnet} learn more discriminative local representations from large scale training data. More recent learning-based matchers, such as SuperGlue~\citep{sarlin2020superglue}, LightGlue~\citep{lindenberger2023lightglue}, and LoFTR~\citep{sun2021loftr}, further improve correspondence estimation by explicitly modeling relationships between local features or directly establishing dense correspondences. These appraoches have substantially improved the robustness of feature matching under challenging appearance and viewpoint changes, leading to stronger performance than traditional structure-based pose estimations. 


% ~\citep{lowe2004distinctive, harris1988combined, rosten2006machine, bay2006surf}. 
% Detected keypoints are then matched through a nearest-neighbor search in the description space.
% In the deep learning era, detectors, descriptors, and matchers can all be replaced by neural networks.
% Most recent works train neural networks for both detectors \cite{yi2016lift,detone2018superpoint,dusmanu2019d2,tyszkiewicz2020disk} and descriptors\cite{mishchuk2017working,tian2019sosnet}.
% In addition, deep-learning-based matchers\cite{sarlin2020superglue,lindenberger2023lightglue,sun2021loftr} can be used to match keypoints generated from neural networks.
% Due to the challenging and large amount of data used for training, these methods provide more versatile features and robust matches, which outperform traditional structure-based pose estimation pipelines.

% \paragraph{Relative Pose Regression}
% Relative pose regression methods directly predict the relative camera pose between image pairs, bypassing the explicit feature matching and geometric estimation stages used in structure-based pipelines~\citep{arnold2022map,ding2019camnet,khatib2024leveraging,zhou2020learn,winkelbauer2021learning,dong2025reloc3r}. These methods aim to learn scene-agnostic geometric representations that generalize across different environments. To improve such generalization, existing approaches are typically trained on large-scale and diverse datasets covering a wide range of indoor and outdoor environments~\citep{laskar2017camera,turkoglu2021visual,dong2025reloc3r}.  

% \textbf{Relative Pose Regression} 
% Relative pose regression methods\cite{arnold2022map,ding2019camnet,khatib2024leveraging,zhou2020learn,winkelbauer2021learning,dong2025reloc3r} regress the relative pose between image pairs, aiming to generalize this capability to different scenes.
% These methods are trained on large and versatile datasets, usually object-centric and include both indoor and outdoor scenes, so that they can adapt to new datasets and scenes\cite{laskar2017camera,turkoglu2021visual,dong2025reloc3r}.
% Relative pose regression methods can be used with multiple query-image pairs, together with triangulation algorithms, to improve the localization and metric-scale estimation\cite{en2018rpnet, arnold2022map, balntas2018relocnet}.

% \paragraph{3D Geometric Foundation Models}
% Recent 3D geometric foundation models~\citep{wang2024dust3r,zhang2024monst3r,fang2025dens3r,leroy2024grounding,wang2025vggt} leverage large-scale 3D datasets~\citep{reizenstein2021common,zhou2018stereo,li2018megadepth,yeshwanth2023scannet++,dehghan2021arkitscenes} to learn generalizable representations of scene geometry. Built largely upon scalable Transformer architectures~\citep{vaswani2017attention}, these models support a broad range of downstream tasks, including 3D reconstruction, geometric perception, spatial reasoning, and camera pose estimation. Large-scale pretraining across diverse scenes and geometric supervision enables them to transfer effectively to previously unseen datasets and environments. DUSt3R~\citep{dust3r_cvpr24} learns dense geometric representations by mapping image pairs into aligned 3D point maps, providing a general purpose representation for downstream 3D tasks. Building upon this paradigm, Relo3r\citep{dong2025reloc3r} adapts a Transformer-based architecture for relative pose regression and directly predicts the relative camera transformation from learned geometric features. This enables pose estimation without explicitly constructing and matching local keypoint correspondences. More recently, VGGT~\citep{wang2025vggt} further demonstrates the potential of large-scale geometric pretraining by jointly predicting multiple scene-level 3D properties, including camera parameters, point maps, depth maps, and 3D point tracks, from one or multiple input images. 

% \textbf{3D Geometric Foundation Models}
% 3D geometric foundation models\cite{wang2024dust3r,zhang2024monst3r,fang2025dens3r,leroy2024grounding,wang2025vggt} are pre-trained neural networks that leverage large-scale 3D data\cite{reizenstein2021common,zhou2018stereo,li2018megadepth,yeshwanth2023scannet++,dehghan2021arkitscenes} and support a diverse array of spatial tasks spanning geometric reconstruction, perception, reasoning, and even generative modeling.
% Due to the scaling ability of the transformer architecture\cite{vaswani2017attention}, these models can generalize well to new datasets, new scenes, and new tasks.
% Reloc3r\cite{dong2025reloc3r} is a transformer-based neural network for relative pose regression, developed upon Dust3r\cite{wang2024dust3r}, a model that is pretrained with a dense 2D to 3D mapping objective.
% They have a shared model architecture, while Reloc3r uses an additional regression head for relative camera pose based on Dust3r features.
% VGGT\cite{wang2025vggt} is a pre-trained neural network that can directly infer all key 3D attributes of a scene, including camera parameters, point maps, depth maps, and 3D point tracks, from one or multiple images.
% Its 3D modeling ability is obtained from large-scale training data with diverse annotations, and simultaneously benefits the camera pose estimation task.

% Existing pose estimators exhibit complementary behavior across different scenes and image pairs, motivating adaptive model selection instead of applying a fixed estimator to every input. 
% \begin{itemize}
%     \item estimator ranking : previous paper shared used that idea to do ranking , but not implemented comprehensively
%     \item pose verification: geometric verification ; learned verification such as FSNet 
% \end{itemize}















% benchmarks for tool use
% merge the VLM two sections 


% \subsection{VLMs for Geometric Vision and Camera Pose Estimation $\to$ waitlist}
% \begin{itemize}
%     \item VLM visual reasoning capabilities
%     \item Prompting-based VLM coding agent $\to$ OpenCV vision tools 
%     \item Fine-tuning VLM $\to$ output geometric results / pose
%     \item VLM's limitaiton
% \end{itemize}


% \subsection{Multimodal Agents and Fallback-driven Tool Use $\to$ waitlist}
% introduce the paradigm of Agent:
% \begin{itemize}
%     \item how do multimodal agent understand visual inputs 
%     \item agent takes external models as tools 
%     \item how to choose and use tool based on task 
%     \item how to use verifier to do fallback and switch to another model
% \end{itemize}




%  VLMs - benchmarks for geometric tasks, there is no models for camera pose estimation for VLMs



% \section{Related Work}

% \paragraph{Relative camera pose estimation.}
% Correspondence-based pipelines detect and match local features and recover the pose with a geometric solver~\citep{multiviewgeometry,lowe2004distinctive,nister2004efficient}, and learned detectors and descriptors~\citep{detone2018superpoint,dusmanu2019d2,tyszkiewicz2020disk}, sparse matchers~\citep{sarlin2020superglue,lindenberger2023lightglue}, and detector-free or dense matchers~\citep{sun2021loftr,edstedt2024roma} have replaced the hand-crafted components. 
% A second line of work obtains the relative pose by network regression rather than from a geometric solver~\citep{arnold2022map,khatib2024leveraging,dong2025reloc3r}, and some of these methods still take matching features as input~\citep{khatib2024leveraging}.
% 3D geometric foundation models~\citep{dust3r_cvpr24,mast3r_eccv24,wang2025vggt} are trained on diverse 3D data to predict scene geometry, and camera poses are either predicted directly or derived from the predicted geometry.
% These lines of work provide candidate estimators with different architectures and output characteristics, and we study how to select among them and verify the poses they return.


==> sections/4analysis.tex <==
\section{Anaslysis of the Best Model for Camera Pose Estimation}
\label{sec:best_model_analysis}

\noindent\textbf{No single pose estimator performs best for every image pair.}
Although recent methods~\citep{lindenberger2023lightglue, edstedt2024roma, dong2025reloc3r, wang2025vggt} have shown improved performance on standard datasets, we found their performance to vary substantially across scenes and individual image pairs.
%
Figure \ref{fig:best freq} reports how frequently each estimator produces the lowest pose error on each dataset, in which the best estimator is determined using the ground truth relative pose.
Reloc3r is selected most frequently on the indoor ARKitScenes~\citep{baruch2021arkitscenes} and ScanNet++~\citep{yeshwanth2023scannet++} datasets, while RoMa Outdoor~\citep{edstedt2024roma} accounts for the largest proportion on MegaDepth~\citep{li2018megadepth} and RealEstate10K~\citep{zhou2018stereo}.
However, even within a single dataset, no estimator consistently performs the best for all image pairs. 
Instead, the best model varies substantially across individual samples.
%

This observation further motivates us to develop an adaptive strategy that selects pose estimators according to characteristics of each input image pair instead of employing a single standalone model.
%
Model performance is affected by image-specific characteristics beyond the coarse indoor and outdoor difference, including viewpoint change, visual overlap, texture, and appearance variation.
%
As a result, an estimator that does not achieve the best overall performance may still provide the most accurate prediction for an image pair. 
%


Based on our analysis, we hypothesize the overall pose accuracy can be improved if one can adaptively select the best model on each image pair.
%
In fact, some correspondence-based methods, such as SuperGlue~\citep{sarlin2020superglue} and RoMa~\citep{edstedt2024roma}, already provide separate model variants for indoor and outdoor scenes, reflecting the fact that a single estimator may not generalize equally well across different visual environments.
%
%Manually selecting between them requires prior knowledge of the scene domain and does not naturally generalize to an arbitrary input image pair.
We introduce \textbf{PoseAgent}, which combines profiling, estimator ranking, and pose verification with orchestration to predict camera pose. 

\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{figures/hist_best_model_per_ds.png}
    \caption{\textbf{Best estimator distribution across datasets.} No single estimator consistently achieves the lowest pose error across all image pairs.}
    % \caption{\textbf{Frequency of each estimator produces the lowest pose error on each dataset.} Although some estimators are selected more frequently on each dataset, no single estimator consistently performs the best across all image pairs.}
    % \caption{The histogram records the frequency of each estimator when it gives the minimum pose error on an image pair. Seven methods are benchmarked on three evaluation datasets.}
    
    \label{fig:best freq}
\end{figure}

% Both traditional and neural network methods rely on an explicit or implicit procedure of keypoint(or image patch) detection, description, and matching.
% However, many real-world scenarios can make this process fail(Figure \ref{fig:Challenging Cases}.
% For example, when an object is moved between two images, the matched keypoints on this object won't follow the same 3D model of the environment, and will result in a wrong solution using 3D geometry.
% Also, if two images are taken in different seasons(Figure \ref{fig:Challenging Cases}: Domain Gap), the description of the same 3D point will be significantly different. Then the matching algorithm will fail to correspond the two points from the two images.
% Besides, if the camera rotates by a large angle, there will be a limited overlapping area between the two images.
% It will be difficult to build the correspondence between the keypoints.
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=1\linewidth]{figures/Challenging Cases.pdf}
%     \caption{Challenging cases for relative camera pose estimation.
%     \textbf{Dynamic scene} makes explicit and implicit keypoint or patch matching algorithms fail to build correspondence.
%     \textbf{Domain gap} makes keypoints or patches features of the same area distant in the feature space, making the matching difficult.
%     \textbf{Large displacement} makes pose estimation rely solely on limited features, which is inherently challenging for both algorithms and humans.}
%     \label{fig:Challenging Cases}
% \end{figure}
% Some keypoint-based methods, such as SuperGlue~\citep{sarlin2020superglue} and RoMa~\citep{edstedt2024roma}, they need to be trained separately on indoor and outdoor datasets.
% Some keypoint-based methods, such as SuperGlue~\citep{sarlin2020superglue} and RoMa~\citep{edstedt2024roma}, provide separate model variants for indoor and outdoor scenes. 
% Although people can manually switch between estimators when dealing with indoor and outdoor samples, this raises the issue of automatic model selection when an arbitrary image pair comes as the input.
% Manually choosing between them requires prior knowledge of the scene domain and does not naturally generalize to an arbitrary input image pair. 
% Meanwhile, there are many other attributes other than indoor and outdoor that can affect the accuracy of every single model.

% Moreover, model performance is affected by image specific characteristics beyond the coarse indoor and ourdoor difference, such as viewpoint change and image appearance.

% Some models might not have the best overall performance, but they can still give the lowest pose error under certain circumstances.

% Therefore, an estimator that might not achieve the best overall performance still can produce the most accurate pose or a particular subset of image pairs. 
% Figure \ref{fig:best freq} reports how frequently each estimator produces the lowest pose error on each dataset, in which the best estimator is identified using the ground truth relative pose. 
% Reloc3r is selected most frequently on the indoor ARKitScenes~\citep{baruch2021arkitscenes} and ScanNet++~\citep{yeshwanth2023scannet++} datasets, while RoMa Outdoor~\citep{edstedt2024roma} accounts for the largest proportion on MegaDepth~\citep{li2018megadepth} and RealEstate10K~\citep{zhou2018stereo}.
% the frequency of each method being the best method on each dataset, where "best" is determined by calculating the pose prediction error based on the ground truth relative camera pose. We observe that Reloc3r dominates in ARKitScenes and ScanNet++ dataset and RoMa (outdoor) performs the best throughout MegaDepth and RealEstate10K. However, it is also obvious that there is not a single model that always is the best one for some images within a dataset.
% However, no estimator consistently performs the best for all image pairs within the same dataste. 
% Instead, the best model varies substantially across individual samples.
% Therefore, the overall prediction accuracy can be improved if one can foresee which estimator will perform the best on each image pair.
% add motivation to seamlessly transit to the next section. 
% show empirical evidence 
% what is the distribution of the datasets -> it doesnot show a single model performs the best all the time 
% put histgrams : for each dataset, which model performs the best. 

==> sections/6experiments_backup.tex <==
\section{Experiments}
% \label{experiments}
% We first introduce the datasets, evaluation metrics, and implementation details in Section \ref{sub:setup}. 
% %
% We then evaluate the overall performace of PoseAgent across four benchmarks against standalone relative pose estimators in Section~\ref{sub:main_results}.
% % 
% This is followed by separate evaluations of the Ranking Agent and Pose Verification Agent in Sections \ref{sub:eval_ranker} and \ref{sub:eval_verifier}, respectively.
% % 
% Next, we compare PoseAgent with prompting-based VLM agents, using Claude Sonnet-5 as the primary baseline, in Section \ref{sub:eval_vlm_agent}.
% %
% Finally, Section~\ref{sub:ablation} presents ablation studies and additional analyses.  

\subsection{Experimental Setup}
\label{sub:setup}
\paragraph{Datasets.} 
We evaluate PoseAgent on four datasets covering both indoor and outdoor environments, including ARKitScenes \citep{baruch2021arkitscenes}, ScanNet++ \citep{yeshwanth2023scannet++}, MegaDepth \citep{li2018megadepth}, and RealEstate10K \citep{zhou2018stereo}. 
%
We follow Reloc3r~\citep{dong2025reloc3r} split for ARKitScenes and the provided split for RealEstate10K, while constructing scene-disjoint training and test splits for MegaDepth and ScanNet++.
%
Across all datasets, the scenes used to train PoseAgent are disjoint from those used for evaluation.
%
Dataset statistics are summarized in Table~\ref{tab:datasets}.
% For ARKitScenes, we sample 20,000 image pairs from the training split adopted by Reloc3r \citep{dong2025reloc3r} and evaluate on its corresponding test set which contains 1,095 image pairs. 
% For RealEstate10K, we similarly sample 20,000 training pairs and evaluate on the provided test set containing 5,449 pairs.
% For MegaDepth, we construct 17,879 training pairs and 2,121 test pairs, While ScanNet++ contains 18,202 training pairs and 1,798 test pairs. 
% For all datasets, the scenes used to train PoseAgent are disjoint from those used for evaluation. 
% For MegaDepth and ScanNet++, both the training and evaluation splits are drawn from scenes included in Reloc3r pretraining, while ARKitScenes and RealEstate10K use the held-out evaluation splits adopted by Reloc3r. 
\input{tables/Datasets for PoseAgent}

\paragraph{Evaluation Metrics.}
We evaluate relative pose estimation using the angular rotation error $e_R$ and translation-direction error $e_t$.
%
For image pair $i$, we define the overall pose error as $e_i = \max(e_{R,i}, e_{t,i})$. 
%
Following prior work~\citep{sarlin2020superglue}, we report the area under the cumulative error curve (AUC) at thresholds of $5\degree$, $10\degree$, and $20\degree$, denoted as AUC@5\degree, AUC@10\degree, and AUC@20\degree, respectively.
% 
Higher AUC values indicate more accurate pose estimates. 

For pose verification, we additionally report the mean Average Accuracy (mAA), following prior work~\citep{barroso2023two, dong2025reloc3r, jin2021image}.
%
We compute mAA@10\degree for rotation, translation, and their maximum error, together with the corresponding median errors~\citep{barroso2023two}.
%
Higher mAA and lower median errors indicate better performance.
% and report the mean Average Accuracy (mAA), obtained by integrating pose accuracy over error thresholds up to $10\degree$. We report $mAA@10\degree$ for rotation, translation, and their maximum pose error, together with the corresponding median rotation, translation, and maximum pose errors~\citep{barroso2023two}. Higher $mAA@10\degree$ and lower median errors indicate better verification performance. 

\paragraph{Implementation Details.} 
We train one ranker and one PVN using data pooled from all four datasets.
%
% We jointly train a single ranker and a single PVN across all four datasets.
Validation pairs are randomly held out from the training scenes, while the test scenes are scene-disjoint from both the training and validation sets.
%

PoseAgent operates over nine candidate estimators, including four SuperGlue variants using indoor or outdoor weights, with or without image resizing (SG-I, SG-O, SG-I-RS, and SG-O-RS)~\citep{sarlin2020superglue}, LightGlue~\citep{lindenberger2023lightglue}, two RoMa variants (RoMa-I and RoMa-O)~\citep{dong2025reloc3r}, Reloc3r~\citep{dong2025reloc3r}, and VGGT~\citep{wang2025vggt}.
%
For SG-I-RS and SG-O-RS, we resize the longer image dimension to 1,600 pixels. 
%
All estimators use their released pretrained weights and default inference configurations.
%
Before verification and evaluation, their predictions are converted to the same camera convention, from camera 1 to camera 2.
% Validation pairs are randomly held out, which test scenes are disjoint from both training and validation scenes. 
% PVN checkpoints are selected by the lowest validation loss. 
% PoseAgent operates over nine candidate relative pose estimators, including SuperGlue-Indoor with image resizing (SG-I-RS)~\citep{sarlin2020superglue}, SuperGlue-Outdoor with image resizing (SG-O-RS), SuperGlue-Indoor (SG-I), SuperGlue-Outdoor (SG-O), LightGlue~\citep{lindenberger2023lightglue}, RoMa-Indoor(RoMa-I)~\citep{edstedt2024roma}, RoMa-Outdoor (RoMa-O), Reloc3r~\citep{dong2025reloc3r}, and VGGT~\citep{wang2025vggt}. 
% For the resized SuperGlue variants, the longer image dimension is resized to 1600 pixels. 
% We use the pretrained weights for all candidate estimators and follow their inference configurations. 
% All predicted relative poses are converted to the same pose convention, from camera 1 to camera 2, before being passed to the ranker and verifier. 

% We implement the Ranking Agent using XGBRanker with the \texttt{rank:ndcg} objective, 300 tree, a maximum depth of 6, and a learning rate of 0.05.
%
% For the PVN, we freeze the pretrained Reloc3r encoder and decoder and train only the newly introduced pose-conditioned modules and pose error prediction heads.
% Training runs for 60 epochs on 7 NVIDIA H100 GPUs using AdamW, with a batch size of 32 per GPU, an initial learning rate of $3\times 10^{-4}$, a weight decay of 0.1, and cosine learning-rate scheduler.

% To increase the diversity of pose candidates, we employ two augmentation strategies. With the probability $p=0.35$, we perturb the original candidate pose. With the probability $q=0.15$, we synthesize a candidate pose around the ground truth pose by independently sampling its rotation and translation-direction. The remaining 50\% of candidates are used without augmentation.  

\subsection{Main Results}
\label{sub:main_results}
% individual models + our methods 
We compare PoseAgent with 9 standalone relative pose estimators across four datasets. 
Each standalone baseline applies a fixed estimator to all image pairs, PoseAgent adaptively ranks candidate estimators and verifies their predictions before producing the final pose estimate.
% Each standalone baseline applies to all image pairs for each dataset. In contrast, PoseAgent ranks the candidate estimators for each image pair and employs a learned verifier to determine whether to accept the current pose estimate or invoke the next ranked estimator. The accepted candidate then outputs the final prediction.
\input{tables/main_results}
As shown in Table~\ref{tab:main_results}, PoseAgent consistently outperforms the strongest estimator across all four datasets and all AUC thresholds.
The gains are particularly pronounced on ScanNet++, where PoseAgent improves AUC@5 from 0.684 to 0.726, and on MegaDepth, where AUC@20 increases from 0.867 to 0.889. 
These results demonstrate that exploiting estimator complementary for arbitrary image pairs yields more robust relative pose estimation than relying on a single fixed estimator.

% As shown in Table \ref{tab:main_results}, PoseAgent consistently outperforms the best standalone estimator in terms of AUC@5, AUC@10, and AUC@20 across all datasets. On the indoor datasets, PoseAgent improves AUC@5 by 1.7\% on ARKitScenes and 4.2\% on ScanNet++. On MegaDepth, an outdoor benchmark, it improves AUC@10 and AUC@20 by 1.7\% ad 2.2\%, respectively. On RealEstate10K, which contains both indoor and outdoor scenes, PoseAgent improves AUC@5, AUC@10, and AUC@20 by 1.2\%, 1.6\%, and 1.6\%, respectively. These consistent improvements demonstrate the benefit of adapting estimator selection and verification to individual image pairs instead of relying on a single fixed estimator. 

\subsection{Evaluation of Ranking Agent}
\label{sub:eval_ranker}
We evaluate whether the proposed ranker can prioritize suitable pose estimators among 9 candidates for each image pair. 
We denote by Rank-$k$, $k \in \{1, ..., 9\}$, the pose estimate produced by the estimator at predicted rank $k$. 
We further report Oracle@$k$, which selects the best pose among Top-$k$ ranked models. 
% Rank-1 and Rank-2 denote the pose estimates produced by the first- and second-ranked estimators, respectively. 

As shown in Table~\ref{tab:eval_ranker}, Rank-1 is competitive with or better than the strongest standalone estimator. The improvement is most evident on ScanNet++ and RealEstate10K, while performance on ARKitScenes and MegaDepth remains comparable to the strongest standalone baselines. 
\input{tables/eval_ranker}

Rank-1 also consistently outperforms Rank-2 across all datasets. 
Figure~\ref{fig:rank_oracle_auc10} shows that Rank-$k$ performance generally decreases with rank, while Oracle@$k$ improves as more candidates are considered. 
This indicates that our ranker produces a meaningful ordering of candidate estimators. 
Oracle@9 provides upper bound, but requires evaluating all candidate estimators. This motivates the verifier introduced in the section~\ref{sub:eval_verifier}, which aims to identify unreliable Rank-1 predictions and selectively fall back to lower-ranked candidates only when necessary.

% Rank-1 achieves competitive performance compared with results from the best standalone estimator. The improvement is most evident on ScanNet++ and RealEstate10K, while performance on ARKitScenes and MegaDepth remains comparable to the strongest standalone baselines. 
% Rank-1 also consistently outperforms Rank-2 across all datasets, indicating that our ranker produces a meaningful ordering of candidate estimators.

% The gap between Rank-1 and Oracle@2 shows that useful alternatives are already present near the top of the ranking. 


\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/rank_oracle_auc10.pdf}
    % \caption{The histogram records the frequency of each estimator when it gives the minimum pose error on an image pair. Seven methods are benchmarked on three evaluation datasets.}
    \caption{\textbf{Performance across predicted estimator rank and oracle top-$k$ selection.} Rank-$k$ reports the AUC@10\degree using the estimator at predicted rank $k$; Oracle@$k$ selects the best prediction among the top-$k$ ranked estimators.}
    \label{fig:rank_oracle_auc10}
\end{figure}

% In this section, we evaluate whether the proposed ranker can identify suitable pose estimator among 9 candidates for each image pair. 
% Their AUC@5/10/20 are calculated by using poses predicted by ranked models. 
% We compare Rank-1 and Rank-2 with results from the best standalone pose estimators on each dataset. We also report AUCs from Oracle@2 and Oracle@9. Oracle@2 selects the better estimates between Rank-1 and Rank2, while Oracle@9 selects the best results from all nine candidates using pose errors. They serve as the upper bounds. 


% As shown in Table \ref{tab:eval_ranker}, Rank-1 achieves competitive performance compared with results from the best standalone models. It improves AUC@5/10/20 most prominent in ScanNet++ and RealEstate10K. In particular, Rank-1 improves AUC@5 from 0.684 to 0.702 on ScanNet++ and AUC@2- from 0.891 to 0.901 on RealEtsate10K. On ARKitScenes and MegaDepth, Rank-1 remains comparable to the best standalone models. These results shows that the ranker can adapt estimator selection to individual image pairs while maintaining or improving the performance of the standalone estimator. 

% Compared with Rank-2 results, Rank-1 consistently outperforms across all datasets. It indicates that the proposed ranker presents a meaningful ranking. Based on results of Oracle@2, it improves Rank-1 results substantially across all datasets. For example, there is still 5.3\%, 2.5\%, 3.7\%, and 3.1\% improvement space at AUC@10 for ARKitScenes, MegaDepth, ScanNet++, and RealEtsate10K, respectively. Oracle@9 establishes a higher upper bound by choosing the best results from all models. However, this requires executing all candidates, leading to more expensive computations. The considerable gap between Rank-1 and Oracle@2 indicates the substantial improvement potential over Rank-1. 

% As a result, these results demonstrate that the ranker successfully prioritize strong candidates but still face challenges to determine the best one through only one round selection. This further motivates our learned verifier, which evaluates the ranked pose candidates and invokes fallback only when the current prediction is considered unreliable.


\subsection{Evaluation of Pose Verification Agent}
\label{sub:eval_verifier}
We evaluate the learned verifier from three complementary perspectives: (1) the accuracy of its predicted pose errors, (2) its ability to select accurate pose hypotheses, and (3) the benefit of our ranking agent compared with fixed ranking order execution and exhaustive verifier-only selection.
% (3) whether ranking agent remains necessary when all candidate poses can be directly verified.

\paragraph{How accurately does the verifier predict pose errors?}
Table~\ref{tab:verifier_mAA_mae} compares our verifier with FSNet~\citep{barroso2023two} using Mean Absolute Error (MAE) over candidate poses for which both methods produce valid predictions.
Our verifier consistently achieves lower MAE for rotation, translation direction, and their maximum pose error. The MAE for the maximum pose decreases from $15.605\degree$ to $4.520\degree$ on ARIkitScenes and from $12.335\degree$ to $2.780\degree$ on RealEstate10K, demonstrating more accurate estimation of candidate pose quality.
% \input{tables/eval_verifier_mae}
\input{tables/eval_verifier_mAA_mae}

\input{tables/eval_verifier_1500}

% We evaluate the learned verifier from three complementary perspectives. 
% First, we measure the accuracy of its predicted pose errors in rotation and translation errors using Mean Absolute Error (MAE). 
% Second, we examine whether these predictions enable reliable selection among multiple pose hypotheses. 
% Finally, we investigate whether the ranker in Subsection~\ref{sub:eval_ranker} remains necessary when the verifier is already allowed to score all 9 pose candidates.

% \paragraph{How accurately does our learned verifier predict pose errors?}
% Table~\ref{tab:verifier_mae} compares the pose error predictions of our verifier with those of FSNet~\citep{loiseau2026alligat0r} over all candidate poses for which both methods produce valid predictions. 
% Our verifier consistently achieves lower MAE for rotation, translation direction, and their maximum on both MegaDepth and ScanNet++.
% On MegaDepth, our verifier reduces MAE of $max(e_R, e_t)$ from $8.588\degree$ to $4.243\degree$.
% The improvement is more pronounced on ScanNet++, in which the MAE of $max(e_R, e_t)$ decreases from $42.854\degree$ to $2.853\degree$. 
% These results demonstrate that our verifier provides substantially more accurate estimates of candidate pose quality.

\paragraph{Can predicted errors reliably select pose hypotheses?}
Following FSNet~\citep{barroso2023two}, we score all 9 candidate poses and select the prediction with the smallest estimated maximum pose error $e_i = max(e_R, e_t)$.
As shown in Table~\ref{tab:verifier_mAA_mae}, our verifier substantially improves pose selection over FSNet on both datasets. 
Despite these improvements, a gap remains between our verifier and the Ground Truth Oracle, which indicates that further improvements are still possible in identifying the best candidate.
% \input{tables/eval_verifier_mAA}

% \paragraph{Can the predicted errors reliably select pose hypotheses?}
% We further investigate whether more accurate error prediction translates into better pose hypotheses selection.
% Following the evaluation approach of FSNet~\citep{barroso2023two}, for each image pair $i$, the verifier scores all 9 candidate poses and selects the one with the smallest predicted maximum pose error $e_i = max(e_R, e_t)$. 
% We evaluate the selected candidate using $\mathrm{mAA}@10\degree$ and median pose errors with respect to the ground truth pose errors for the selected candidate.

% As shown in Table~\ref{tab:eval_verifier_mAA}, our learned verifier substantially outperforms FSNet in both $\mathrm{mAA}@10\degree$ and median pose errors from 0.655 to 0.839 on MegaDepth and from 0.284 to 0.904 on ScanNet++.
% Despite these improvements, a gap remains between our verifier and the GT oracle, indicating that selecting hypotheses solely based on the best predicted errors still needs further improvement. 

% % \paragraph{Is the ranking agent still necessary?}
% Because predicted pose errors naturally induce a ranking over candidate poses, we further compare among verifier-only selection, the ranking agent, and the complete PoseAgent in Table~\ref{tab:comp_verifier_only}.
% Verifier-only selection, which exhausts all candidate poses, does not consistently outperform Rank-1. 
% It performs better on ScanNet++, but worse on ARKitScenes and RealEstate10K. 
% In contrast, PoseAgent, which combines ranking agent and verification agent, achieves the strongest overall performance.
% These results suggest that the two components are complementary. The ranking agent prioritizes estimators based on image profiling features, while the verifier assesses the reliability of the resulting pose predicitons.
\paragraph{Does ranking agent improve pose selection?}
We compare four selection strategies in Table~\ref{tab:comp_verifier_only}, including verifier-only selection over all nine candidates, ranker-only selection using the top-ranked estimator, a fixed-order baseline with PVN, and the complete PoseAgent. 

For the fixed-order baseline, we sort estimators by their average win rate across the four training datasets, weighting each dataset equally. 
The resulting order is shared by all test pairs. 
This baseline uses the same PVN, verification thresholds, fallback policy, maximum number of models executed ($K$ = 4) as PoseAgent.

PoseAgent outperforms the fixed-order baseline across all four datasets and all AUC@5/10/20. These results demonstrate the benefit of ranking agent over a fixed order based on prior winning distribution within the same verification and fallback framework.

Compared with verifier-only selection, PoseAgent achieves higher AUC on three datasets, while verifier-only selection remains slightly better on ScanNet++. Together, these comparisons support the complementary understanding of ranking agent and verification, without requiring exhaustive execution of all nine estimators. 
\input{tables/eval_verifier_ranker+verifier}

% Because the verifier predicts pose errors of individual pose candidates, its predictions naturally induce a ranking over the available candidates. 
% Indeed, FSNet~\citep{barroso2023two} uses predicted pose errors to score and select among multiple hypotheses. This raises a natural question: \textit{if all 9 estimators can be executed and their predictions verified, is our proposed ranker still necessary?}
% Table~\ref{tab:comp_verifier_only} shows that verifier-only selection does always outperform Ranker Top-1. Although it performs better on ScanNet++, it performs worse on ARKitScenes and RealEstate10K. These results suggest that directly selecting the minimum among multiple error predictions is not always optimal. 
% The ranker in Subsection~\ref{sub:eval_ranker} provides a complementary prior by prioritizing models that are more suitable for each image pair before their pose predictions are verified. 
% This complementary is demonstrated by PoseAgent, which combines the learnable ranker with verification guided selection and fallback. 
% As shown in the third row of Table~\ref{tab:comp_verifier_only}, PoseAgent achieves the strongest performance on ARkitScenes, MegaDepth, and RealState10K, while remaining within 0.2\% of verifier-only selection on ScanNet++.
% In addition, PoseAgent consistently improves over Ranker Top-1 across all reported dataset. 

% Overall, our learned verifier predicts candidate pose errors more accurately than FSNet and selects more accurate pose hypotheses. 
% However, ranking all candidates solely by their predicted errors is always not optimal. It does not eliminate the necessity of the ranker. Instead, the two components provide complementary information. The ranker supplies an input information over estimator suitability, while the verifier further assesses the reliability of the resulting pose estimates.  



% \textbf{Is our ranker still necessary, if our verifier can be used to select the potential hypotheses?}
% Because verifiers predict pose errors in rotation and translation, it naturally induce a ranking over candidate poses. This is also how FSNet \citep{barroso2023two} scores from multiple hypotheses and get the best candidate based on the predicted pose errors. We further ask whether our proposed ranker is still necessary when all nine models can be executed with pose errors predicted. Table \ref{tab:comp_verifier_only} shows that the learned verifier-only selection does not consistently outperform Ranker Top-1. It performs better on ScanNet++ but is inferior on ARKitScenes, MegaDepth, and RealEstate10K. This suggests that solely relying on the verifier to select the hypothesis with the most minimal pose errors is not sufficient. However, the introduction of ranker to the learned verifier can provide a complementary prior for model selection. It is also evidenced by the 3rd row in Table \ref{tab:comp_verifier_only}, PoseAgent: Ranker + Verifier, in which the combination of two components produces the strongest performance on ARkitScenes, MegaDepth, and RealState10K, while remaining within 0.1\% difference on ScanNet++. 

% Overall, our verifier predicts candidate errors more accurately than FSNet and selects better pose hypotheses. However, verifier-only ranking over all candidates does not eliminate the need for the ranker.

% Verifier vs. FSNet

\subsection{Comparison with VLM-Based Agents}
\label{sub:eval_vlm_agent}
% claude (OpenCV), VLM + our own verfifer, our pipeline 
We conduct the VLM-based evaluation on the ARKitScenes test set. We consider three prompting-based settings:
(1) a VLM coding agent that generates and executes pose estiamtion pipelines;
(2) a VLM ranker that takes the profiling features of each image pair and ranks the 9 candidate pose estimators;
(3) the VLM ranker combined with our learned verifier and fallback policy. 
We use \textbf{Claude Sonnet-5} in all VLM-based experiments. 
The results lead to the following findings. 


% We conduct the VLM-based evaluation on the ARKitScenes test set. We consider three prompting-based settings: (1) VLM coding agent that generates and executes pose estimation, (2) VLM as a ranker that takes each image pair's profiling features and ranks 9 pose estimators, and (3) VLM as a ranker combined with our learned verifier and fallback policy. We use \textbf{Claude Sonnet-5} for all VLM-based experiments and apply the same evaluation convention and candidate pose estimates as those used for PoseAgent. 

% Based on these three settings, we aim to answer the following two questions:

\paragraph{VLM coding agents remain limited for accurate pose estimation.}
As shown in Table~\ref{tab:comp_vlm_agent}, the VLM coding agent constructs and executs an OpenCV-based geometric pipeline, but falls substantially behind PoseAgent. This suggests that generating executable pipelines alone does not ensure accurate relative pose estimation in our setting. 
% Table~\ref{tab:comp_vlm_agent} compares PoseAgent with a prompting-based VLM coding agent on ARKitScenes. Although the VLM agent can generate and execute an OpenCV-based geometric estimation pipeline, it achieves only 0.090/0.163/0.259 in AUC@5/10/20. In contrast, PoseAgent achieves 0.473/0.685/0.823. These results indicates that, under our experimental setting, VLM code generation and conventional geometric tool use alone are insufficient for reliable relative pose estimation. 
\input{tables/comparison_VLM_agents}

% \paragraph{How is VLM coding agent for pose estimation?}
% Table~\ref{tab:comp_vlm_agent} compares PoseAgent with a prompting-based VLM coding agent on ARKitScenes. Although the VLM agent can generate and execute an OpenCV-based geometric estimation, it achieves only 0.090/0.163/0.259 in AUC@5/10/20. In contrast, PoseAgent achieves 0.473/0.685/0.823, indicating that current VLM coding agent is still confined to basic OpenCV code generation and tool use. This is still not sufficient for more accurate pose estimation. Substantial gains are obtained by equipping the agent with different pose estimators, image-tailored ranking and pose verification. 

\paragraph{Ranking Agent outperforms VLM-based ranking.}
Our ranker consistently outperforms the VLM ranker in both Top-1 and Oracle@2 evaluations, as shown in Table~\ref{tab:vlm_as_ranker}, indicating stronger initial selection and better coverage of suitable estimators within the top two candidates.
\input{tables/vlm_as_ranker}
% Table~\ref{tab:vlm_as_ranker} shows that our learnable ranker substantially outperforms the VLM ranker under both Top-1 and Oracle@2 evaluation. For Top-1 selection, our ranker improves AUC@5/10/20 by 9.1/12.5/12.5\%. Under Oracle@2, Our ranker's performance surpasses VLM substantially. This indicates that our ranker not only selects a stronger top-1 candidate but also places most suitable estimators near the top of its ordering. 


% \paragraph{How accurately does VLM as a ranker?}
% Additionally, we further use VLM as a ranker to output ranked candidate models by taking profiling features for a specific image pair. Table~\ref{tab:vlm_as_ranker} shows that our ranker surpasses the VLM-based ranking under both Top-1 and Oracle@2 evaluation. It not only selects a stronger first candidate but also places higher quality estimators near the top of the ranking. 

\paragraph{Verification improves VLM ranking.} 
Augmenting the VLM ranker with our learned verifier and fallback policy substantially improves accuracy, as shown in Table~\ref{tab:vlm_as_ranker}. With the same verification and fallback policy and a maximum of four candidates, PoseAgent still performs better, highlighting the complementary contributions of learned ranking agent and verification. 
% Under the same configuration of verifier and fallback policy as well as the maximum rank of top 4 models, combining the ranking results generated by VLM with our learned verifier and fallback policy improves AUC@5/10/20 from 0.369/0.549/0.691 to 0.449/0.650/0.795. Furthermore, PoseAgent further improves these results. These results show that verification can further correct VLM ranking and learnabled ranking remains more reliable.  



% We further apply our verifier and fallback policy to the VLM ranker. The fallback policy sequentially takes Top-4 candidates to determine whether accept or verify the next candidate until it exhausts top-4 models. Table~\ref{tab:vlm_as_ranker} shows the integration with the VLM ranker and our verifier, following the same fallback policy, improves the results of VLM ranker only. Furthermore, PoseAgent still consistently outperforms VLM Ranker + Verifier by 2.4 -- 3.5\%. 

\subsection{Ablation Studies}
\label{sub:ablation}
% ranker alone vs. ranker + verifier 
% best working results 
% how many iteration (top-K) 
% \subsubsection{Effect of verifier augmentation/threshold/top-k}
\subsubsection{Effect of profiling features}
We first examine how different profiling features affect estimator ranking. \textit{Scene features} use the predicted scene types of two input images. 
\textit{Geometry features} correspondence, overlap, keypoint distribution, motion, and geometric consistency features. 
\textit{All features} use all profiling features. 
We keep the same configuration for each ranker, PVN, verification thresholds, and the fallback policy as well as the maximum number of estimators ($K$=4).

As shown in Table~\ref{tab:profiling_ablation}, \textit{Geometry features} outperforms \textit{Scene features} across all four datasets on AUC@5/10/20\degree. 
Although coarse scene type information alone already achieves good results, they are still insufficient to account for the performance of PoseAgent. 
\textit{Geometry features} matches \textit{All features} on ARKitScenes and ScanNet++, while \textit{All features} result provides modest, consistent improvements on the other datasets. 
These results suggest that geometric profiling features further supply additional information needed for effective esitmator ranking.

\input{tables/profiling_ablation}

\subsubsection{Effect of maximum number of estimators used}
We change the maximum number of estimator executed ($K$) from 1 to 6, with ($\tau_R=0.5^\circ$) and ($\tau_t=6^\circ$) fixed. 
As shown in Figure~\ref{fig:ablation_topK}, allowing fallback beyond the top-ranked estimator improves performance across all four datasets and all three AUC thresholds. 
Most gains are obtained withint he first few candidates. 
Further increasing ($K$) yields diminishing gains on ScanNet++. It als can reduce accuracy on the other datasets, indicating that evaluating more candidates does not necessarily improve final selection. We use ($k$ = 4) as a final maximum number of models. 

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/ablation_top-k.pdf}
    % \caption{The histogram records the frequency of each estimator when it gives the minimum pose error on an image pair. Seven methods are benchmarked on three evaluation datasets.}
    \caption{\textbf{Effect of the execution budget on relative pose accuracy.} We report AUC@5/10/20\degree as the maximum number of estimator executions $K$ varies, with $\tau_R=0.5^\circ$ and $\tau_t=6^\circ$ fixed. Dashed lines indicate the current setting, $K=4$.}
    \label{fig:ablation_topK}
\end{figure}

\subsubsection{Inference Latency Analysis}
\input{tables/latency}


% \subsubsection{Analysis of backbone pretraining bias}
% Since our verifier uses a frozen Reloc3r encoder-decoder backbone, whose pretraining data include several datasets used in our experiments, we further examine whether the reported gains could be explained by representation level exposure or esitimator-specific bias. 

% \paragraph{Does the verifier generalize beyond Reloc3r-pretraining-exposed scenes?}
% As shown in Table~\ref{tab:verifier_mae}, our verifier consistently outperforms FSNet not only on MegaDepth and ScanNet++, whose evaluation scenes are drawn from Reloc3r pretraining scenes, but also on the held-out ARKitScenes and RealEstate10K evaluation splits.
% This indicates that the improvements is not restricted to scenes exposed during Reloc3r pretraining. 

% \paragraph{Does the verifier favor Reloc3r generated poses?}
% We next evaluate verifier accuracy separately based on candidate estimators, using the common subset of image pairs for which all nine estimators produce valid predictions. Although Reloc3r-generated poses exhibit relatively low raw MAE on several datasets, this advantage is not universal across datasets or error components, indicating that 

% \paragraph{Does the verifier still favor Reloc3r after controlling for candidate difficulty?}
% \paragraph{Reloc3r backbone vs. another frozen backbone / randomly initialized verifier backbone}
% or: remove reloc3r candidates from the estimator pool and reevaluate the verifier 


% 可以consider的
% ranker-only
% ranker + fallback 
% ranker + FSNet Verifier + Fallback 
% ranker + learned Verifier + Fallback 
% Full PoseAgent
% profiling features ? 
% 不同的Top-K
% verification thresholds 
% accuracy-runtime trade-off





% \subsection{Comparison with VLM-based Approaches}
% \begin{itemize}
%     \item Fine-tuning VLM
%     \item VLM Coding Agent by prompting
% \end{itemize}

% \subsection{Comparison with Individual Pose Estimators}
% \begin{itemize}
%     \item 9 individual pose results vs. final results (after verification)
% \end{itemize}
% metrics 
% quantitive results 
% visualization


% \section{Headings: first level}
% \label{headings}

% First level headings are in small caps,
% flush left and in point size 12. One line space before the first level
% heading and 1/2~line space after the first level heading.

% \subsection{Headings: second level}

% Second level headings are in small caps,
% flush left and in point size 10. One line space before the second level
% heading and 1/2~line space after the second level heading.

% \subsubsection{Headings: third level}

% Third level headings are in small caps,
% flush left and in point size 10. One line space before the third level
% heading and 1/2~line space after the third level heading.

==> sections/7results.tex <==
% \section{Ablation}
% \label{ablation}



% \subsection{Effect of Ranker}
% \begin{itemize}
%     \item results of VLM as a ranker vs. ours
% \end{itemize}

% \subsection{Effect of Verifier}
% \begin{itemize}
%     \item results of ranking vs. results of verifier 
%     \item results of FSNet vs. our results 
% \end{itemize}

% \subsection{Unified Rule for Fallback Policy}
% \begin{itemize}
%     \item Different Top-K

% \end{itemize}

% \section{Conclusion}

\section{Example Visualization}
\label{example_visualization}
We show the execution behavior of PoseAgent on selected test pairs. 
For each image pair, we show the predicted estimator ordering, the candidates actually executed, the pose errors predicted by PAV, and the resulting acceptance or fallback decisions. 

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/example1_viz.pdf}
    % \caption{The histogram records the frequency of each estimator when it gives the minimum pose error on an image pair. Seven methods are benchmarked on three evaluation datasets.}
    \caption{}
    \label{fig:exp1_viz}
\end{figure}



==> tables/eval_ranker.tex <==
%define colors
\definecolor{rankerbg}{RGB}{255, 226, 153} % light yellow 
\definecolor{verifierbg}{RGB}{252, 229, 205} % light pink 
\definecolor{numred}{RGB}{255, 0, 0}
\definecolor{numgreen}{RGB}{112, 173, 71}
\definecolor{numblue}{RGB}{0, 0, 255}
\definecolor{lightgray}{gray}{0.9}

% \begin{table*}[t]
%     \centering
%     % \caption{\textbf{Performance of learnable ranker and its oracle upper bounds.} \textcolor{numred}{Red} and \textcolor{numblue}{blue} represents the better results from Rank-1 model and results from the best standalone estimator, respectively. Oracle@2 is calculated by choosing the best results from rank-1 and rank-2 estimators. Oracle@9 is calculated based on the best results from all 9 candidate estimators.}
%     % \caption{\textbf{Performance of ranking agent and oracle upper bounds.} Rank-1 and Rank-2 denote predictions from the first- and second-ranked estimators. Oracle@2 selects the better of Rank-1 and Rank-2 pose error, while Oracle@9 selects the best among all candidates.}
%     % \caption{\textbf{Performance of ranking agent and oracle upper bounds.} Rank-1 and Rank-2 denote predictions from the first- and second-ranked estimators. Oracle@2 selects the better of Rank-1 and Rank-2 pose error.}
%     \caption{\textbf{Ranking performance across four datasets.} }
    
%     \label{tab:eval_ranker}
%     \footnotesize
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{lcccccccccccc}
%         \toprule

%         & \multicolumn{3}{c}{\textbf{ARKitScenes}}
%         & \multicolumn{3}{c}{\textbf{MegaDepth}}
%         & \multicolumn{3}{c}{\textbf{ScanNet++}}
%         & \multicolumn{3}{c}{\textbf{RealEstate10K}} \\

%         \cmidrule(lr){2-4}
%         \cmidrule(lr){5-7}
%         \cmidrule(lr){8-10}
%         \cmidrule(lr){11-13}

%         \textbf{Method}
%         & \textbf{@5\degree} & \textbf{@10\degree} & \textbf{@20\degree}
%         & \textbf{@5\degree} & \textbf{@10\degree} & \textbf{@20\degree}
%         & \textbf{@5\degree} & \textbf{@10\degree} & \textbf{@20\degree}
%         & \textbf{@5\degree} & \textbf{@10\degree} & \textbf{@20\degree} \\
%         \midrule

%         % Best Standalone
%         % & 0.456	& \underline{0.675} & \underline{0.819}
%         % & \underline{0.684}	& 0.793	& 0.867	
%         % & 0.684	& 0.833	& 0.915	
%         % & 0.724	& 0.827	& 0.891 \\

%         Rank-1
%         & {\bf 0.460}	& 0.674	& 0.816	
%         & 0.682	& {\bf 0.794}	& {\bf 0.869}
%         & {\bf 0.702} & {\bf 0.839} & {\bf 0.916}
%         &  {\bf 0.729}	&  {\bf 0.836}	& {\bf 0.901} \\
        

%         Rank-2
%         & 0.393	& 0.591	& 0.742	
%         & 0.655	& 0.774	& 0.855	
%         & 0.543	& 0.680	& 0.779	
%         & 0.682	& 0.805	& 0.882 \\
        
%         \midrule
%         \rowcolor{lightgray}
%         Oracle@2
%         & 0.532	& 0.727	& 0.851	
%         & 0.715	& 0.819	& 0.888	
%         & 0.762	& 0.876	& 0.937	
%         & 0.774	& 0.867	& 0.921 \\ 

%         % \rowcolor{lightgray}
%         % Oracle@9
%         % & 0.607	& 0.778	& 0.881	
%         % & 0.803	& 0.888	& 0.940	
%         % & 0.800	& 0.897	& 0.948	
%         % & 0.829	& 0.900	& 0.941 \\
        

        

%         % \rowcolor{rankerbg}
%         % \midrule
%         % \textbf{Ranker} (Ours)
%         % & \textcolor{numgreen}{0.460}	& 0.674	& 0.816	
%         % & 0.682	& \textcolor{numgreen}{0.794}	& \textcolor{numgreen}{0.869}
%         % & \textcolor{numgreen}{0.702}	& \textcolor{numgreen}{0.839}	& \textcolor{numgreen}{0.916}
%         % & \textcolor{numgreen}{0.729}	& \textcolor{numgreen}{0.836}	& \textcolor{numgreen}{0.901} \\


%         \bottomrule
%     \end{tabular}
    
%     }
% \end{table*}

% Table 3
\begin{table}[t]
    \centering
    \caption{\textbf{Ranking performance across four datasets.} Results are AUC@5\degree/10\degree/20\degree. }
    \label{tab:eval_ranker}
    \scriptsize
    \setlength{\tabcolsep}{4pt}
    \renewcommand{\arraystretch}{0.95}
    \begin{tabular}{lcccc}
        \toprule
        \textbf{Method}
        & \textbf{ARKitScenes}
        & \textbf{MegaDepth}
        & \textbf{ScanNet++}
        & \textbf{RealEstate10K} \\
        \midrule
        Rank-1
        & \textbf{0.460 / 0.674 / 0.816}
        & \textbf{0.682 / 0.794 / 0.869}
        & \textbf{0.702 / 0.839 / 0.916}
        & \textbf{0.729 / 0.836 / 0.901} \\

        Rank-2
        & 0.393 / 0.591 / 0.742
        & 0.655 / 0.774 / 0.855
        & 0.543 / 0.680 / 0.779
        & 0.682 / 0.805 / 0.882 \\
        \midrule

        \rowcolor{gray!10}
        Oracle@2
        & 0.532 / 0.727 / 0.851 
        & 0.715 / 0.819 / 0.888 
        & 0.762 / 0.876 / 0.937 
        & 0.774 / 0.867 / 0.921 \\
        \bottomrule
    \end{tabular}
\end{table}




==> tables/eval_verifier_mAA.tex <==
\begin{table*}[t]
    \centering
    \small
    \caption{
        \textbf{Pose selection using predicted pose errors.}
        Higher mAA@10$^\circ$ and lower median error indicate better selection.
        GT Oracle selects the best candidate using ground-truth pose error.
    }
    \label{tab:eval_verifier_mAA}
    \vspace{4pt}

    % ==================== ARKitScenes ====================
    % \begin{minipage}[t]{0.49\textwidth}
    %     \centering
    %     \textbf{\strut ARKitScenes}
    %     \vspace{1mm}

    %     \resizebox{\linewidth}{!}{
    %         \begin{tabular}{lcccccc}
    %             \toprule
    %             & \multicolumn{3}{c}{\textbf{mAA@10$^\circ$} $\uparrow$}
    %             & \multicolumn{3}{c}{\textbf{Median Error ($^\circ$)} $\downarrow$} \\
    %             \cmidrule(lr){2-4}
    %             \cmidrule(lr){5-7}

    %             \textbf{Method}
    %             & $\mathbf{e_R}$
    %             & $\mathbf{e_t}$
    %             & $\mathbf{e_{\max}}$
    %             & $\mathbf{e_R}$
    %             & $\mathbf{e_t}$
    %             & $\mathbf{e_{\max}}$ \\
    %             \midrule

    %             FSNet
    %             & 0.738
    %             & 0.467
    %             & 0.440
    %             & 1.802
    %             & 5.030
    %             & 5.463 \\

    %             \rowcolor{gray!10}
    %             \textbf{Ours}
    %             & \textbf{0.920}
    %             & \textbf{0.738}
    %             & \textbf{0.716}
    %             & \textbf{0.839}
    %             & \textbf{2.007}
    %             & \textbf{2.332} \\

    %             \midrule

    %             \textit{GT Oracle}
    %             & 0.945
    %             & 0.843
    %             & 0.827
    %             & 0.670
    %             & 1.306
    %             & 1.502 \\

    %             \bottomrule
    %         \end{tabular}
    %     }
    % \end{minipage}
    % \hfill
    % ==================== ScanNet++ ====================
    \begin{minipage}[t]{\textwidth}
        \centering
        \small
        \textbf{\strut ScanNet++}
        % \vspace{1mm}

        \resizebox{\linewidth}{!}{
            \begin{tabular}{lcccccc}
                \toprule
                & \multicolumn{3}{c}{\textbf{mAA@10$^\circ$} $\uparrow$}
                & \multicolumn{3}{c}{\textbf{Median Error ($^\circ$)} $\downarrow$} \\
                \cmidrule(lr){2-4}
                \cmidrule(lr){5-7}

                \textbf{Method}
                & $\mathbf{e_R}$
                & $\mathbf{e_t}$
                & $\mathbf{e_{\max}}$
                & $\mathbf{e_R}$
                & $\mathbf{e_t}$
                & $\mathbf{e_{\max}}$ \\
                \midrule

                FSNet
                & 0.462
                & 0.340
                & 0.284
                & 5.311
                & 10.005
                & 13.978 \\

                \rowcolor{gray!10}
                \textbf{Ours}
                & \textbf{0.958}
                & \textbf{0.928}
                & \textbf{0.904}
                & \textbf{0.599}
                & \textbf{0.712}
                & \textbf{1.034} \\

                \midrule

                \textit{GT Oracle}
                & 0.972
                & 0.958
                & 0.942
                & 0.416
                & 0.541
                & 0.712 \\

                \bottomrule
            \end{tabular}
        }
    \end{minipage}

    \vspace{3mm}

    % ==================== MegaDepth ====================
    \begin{minipage}[t]{\textwidth}
        \centering
        \textbf{\strut MegaDepth}
        \vspace{1mm}

        \resizebox{\linewidth}{!}{
            \begin{tabular}{lcccccc}
                \toprule
                & \multicolumn{3}{c}{\textbf{mAA@10$^\circ$} $\uparrow$}
                & \multicolumn{3}{c}{\textbf{Median Error ($^\circ$)} $\downarrow$} \\
                \cmidrule(lr){2-4}
                \cmidrule(lr){5-7}

                \textbf{Method}
                & $\mathbf{e_R}$
                & $\mathbf{e_t}$
                & $\mathbf{e_{\max}}$
                & $\mathbf{e_R}$
                & $\mathbf{e_t}$
                & $\mathbf{e_{\max}}$ \\
                \midrule

                FSNet
                & 0.850
                & 0.683
                & 0.655
                & 0.835
                & 1.867
                & 2.185 \\

                \rowcolor{gray!10}
                \textbf{Ours}
                & \textbf{0.964}
                & \textbf{0.850}
                & \textbf{0.839}
                & \textbf{0.393}
                & \textbf{0.814}
                & \textbf{1.017} \\

                \midrule

                \textit{GT Oracle}
                & 0.983
                & 0.931
                & 0.928
                & 0.236
                & 0.390
                & 0.483 \\

                \bottomrule
            \end{tabular}
        }
    \end{minipage}
    \hfill
    % ==================== RealEstate10K ====================
    % \begin{minipage}[t]{0.49\textwidth}
    %     \centering
    %     \textbf{\strut RealEstate10K}
    %     \vspace{1mm}

    %     \resizebox{\linewidth}{!}{
    %         \begin{tabular}{lcccccc}
    %             \toprule
    %             & \multicolumn{3}{c}{\textbf{mAA@10$^\circ$} $\uparrow$}
    %             & \multicolumn{3}{c}{\textbf{Median Error ($^\circ$)} $\downarrow$} \\
    %             \cmidrule(lr){2-4}
    %             \cmidrule(lr){5-7}

    %             \textbf{Method}
    %             & $\mathbf{e_R}$
    %             & $\mathbf{e_t}$
    %             & $\mathbf{e_{\max}}$
    %             & $\mathbf{e_R}$
    %             & $\mathbf{e_t}$
    %             & $\mathbf{e_{\max}}$ \\
    %             \midrule

    %             FSNet
    %             & 0.830
    %             & 0.621
    %             & 0.607
    %             & 0.964
    %             & 2.846
    %             & 3.062 \\

    %             \rowcolor{gray!10}
    %             \textbf{Ours}
    %             & \textbf{0.942}
    %             & \textbf{0.875}
    %             & \textbf{0.865}
    %             & \textbf{0.314}
    %             & \textbf{0.888}
    %             & \textbf{0.995} \\

    %             \midrule

    %             \textit{GT Oracle}
    %             & 0.967
    %             & 0.942
    %             & 0.940
    %             & 0.182
    %             & 0.410
    %             & 0.441 \\

    %             \bottomrule
    %         \end{tabular}
    %     }
    % \end{minipage}
\end{table*}

% \begin{table*}[t]
%     \centering
%     \caption{Relative pose estimation results. Higher is better for mAA@10$^\circ$, while lower is better for median error.}
%     \label{tab:eval_verifier_mAA}
%     \vspace{10pt}
%     % ==================== ARKitScenes ===================
%     \begin{minipage}[t]{0.49\textwidth}
%         \centering
%         \textbf{\strut ARKitScenes}
%         \vspace{1mm}

%         \resizebox{\linewidth}{!}{
%         \begin{tabular}{lcccccc}
%             \toprule
%             & \multicolumn{3}{c}{\textbf{mAA@10$^\circ$} $\uparrow$}
%             & \multicolumn{3}{c}{\textbf{Median ($^\circ$)} $\downarrow$} \\
%             \cmidrule(lr){2-4}
%             \cmidrule(lr){5-7}

%             \textbf{Method}
%             & \textbf{R}
%             & \textbf{t}
%             & $\mathbf{\max(R,t)}$
%             & \textbf{$e_R$}
%             & \textbf{$e_t$}
%             % & $\mathbf{\max(e_R,e_t)}$ \\
%             & $e_{\max}$ \\ 
%             \midrule

%             FSNet
%             & 0.738 & 0.467 & 0.440 
%             & 1.802 & 5.030 & 5.463\\

%             \rowcolor{gray!12}
%             \textbf{Verifier (PoseAgent)}
%             & 0.920	& 0.738	& 0.716
%             & 0.839	& 2.007	& 2.332 \\

%             \midrule
            
%             \rowcolor{gray!7}
%             GT Oracle
%             & 0.945	& 0.843	& 0.827
%             & 0.670	& 1.306	& 1.502 \\

%             \bottomrule
%         \end{tabular}
%         }
%     \end{minipage}
%     \hfill
    
%     % ==================== MegaDepth ====================
%     \begin{minipage}[t]{0.49\textwidth}
%         \centering
%         \textbf{\strut MegaDepth}
%         \vspace{1mm}

%         \resizebox{\linewidth}{!}{
%         \begin{tabular}{lcccccc}
%             \toprule
%             & \multicolumn{3}{c}{\textbf{mAA@10$^\circ$} $\uparrow$}
%             & \multicolumn{3}{c}{\textbf{Median ($^\circ$)} $\downarrow$} \\
%             \cmidrule(lr){2-4}
%             \cmidrule(lr){5-7}

%             \textbf{Method}
%             & \textbf{R}
%             & \textbf{t}
%             & $\mathbf{\max(R,t)}$
%             & \textbf{$e_R$}
%             & \textbf{$e_t$}
%             % & $\mathbf{\max(e_R,e_t)}$ \\
%             & $e_{\max}$ \\ 
%             \midrule

%             FSNet
%             & 0.850	& 0.683	& 0.655	
%             & 0.835	& 1.867	& 2.185 \\

%             \rowcolor{gray!12}
%             \textbf{Verifier (PoseAgent)}
%             & {\bf 0.964}	& {\bf 0.850}	& {\bf 0.839}
%             & {\bf 0.393}	& {\bf 0.814}	& {\bf 1.017} \\

%             \midrule
            
%             \rowcolor{gray!7}
%             GT Oracle
%             & 0.983	& 0.931	& 0.928	
%             & 0.236	& 0.390	& 0.483 \\

%             \bottomrule
%         \end{tabular}
%         }
%     \end{minipage}
%     \hfill
%     % ==================== ScanNet ====================
%     \begin{minipage}[t]{0.49\textwidth}
%         \centering
%         \textbf{\strut ScanNet++}
%         \vspace{1mm}

%         \resizebox{\linewidth}{!}{
%         \begin{tabular}{lcccccc}
%             \toprule
%             & \multicolumn{3}{c}{\textbf{mAA@10$^\circ$} $\uparrow$}
%             & \multicolumn{3}{c}{\textbf{Median ($^\circ$)} $\downarrow$} \\
%             \cmidrule(lr){2-4}
%             \cmidrule(lr){5-7}

%             \textbf{Method}
%             & \textbf{R}
%             & \textbf{t}
%             & $\mathbf{\max(R,t)}$
%             & \textbf{$e_R$}
%             & \textbf{$e_t$}
%             % & $\mathbf{\max(e_R,e_t)}$ \\
%             & $e_{\max}$ \\

%             \midrule

%             FSNet
%             & 0.462	& 0.340	& 0.284	
%             & 5.311	& 10.005 & 13.978 \\

%             \rowcolor{gray!12}
%             \textbf{Verifier (PoseAgent)}
%             & {\bf 0.958}	& {\bf 0.928}	& {\bf 0.904}
%             & {\bf 0.599}	& {\bf 0.712}	& {\bf 1.034} \\

%             \midrule
%             \rowcolor{gray!7}
%             GT Oracle
%             & 0.972	& 0.958	& 0.942	
%             & 0.416	& 0.541	& 0.712 \\

%             \bottomrule
%         \end{tabular}
%         }
%     \end{minipage}


%     % ==================== RealEstate10K ====================
%     \begin{minipage}[t]{0.49\textwidth}
%         \centering
%         \textbf{\strut RealEstate10K}
%         \vspace{1mm}

%         \resizebox{\linewidth}{!}{
%         \begin{tabular}{lcccccc}
%             \toprule
%             & \multicolumn{3}{c}{\textbf{mAA@10$^\circ$} $\uparrow$}
%             & \multicolumn{3}{c}{\textbf{Median ($^\circ$)} $\downarrow$} \\
%             \cmidrule(lr){2-4}
%             \cmidrule(lr){5-7}

%             \textbf{Method}
%             & \textbf{R}
%             & \textbf{t}
%             & $\mathbf{\max(R,t)}$
%             & \textbf{$e_R$}
%             & \textbf{$e_t$}
%             % & $\mathbf{\max(e_R,e_t)}$ \\
%             & $e_{\max}$ \\ 
%             \midrule

%             FSNet
%             & 0.830	& 0.621	& 0.607	
%             & 0.964	& 2.846	& 3.062 \\

%             \rowcolor{gray!12}
%             \textbf{Verifier (PoseAgent)}
%             & 0.942	& 0.875	& 0.865	
%             & 0.314	& 0.888	& 0.995 \\

%             \midrule
            
%             \rowcolor{gray!7}
%             GT Oracle
%             & 0.967	& 0.942	& 0.940	
%             & 0.182	& 0.410	& 0.441 \\

%             \bottomrule
%         \end{tabular}
%         }
%     \end{minipage}
%     \hfill

% \end{table*}

==> tables/eval_verifier_mae.tex <==
\begin{table}[t]
    \centering
    % \caption{\textbf{Mean absolute error (MAE) comparison.} MAE is compared over all common valid pose candidates from MegaDepth and ScanNet++ for FSNet and our learned verifier.}
    \caption{\textbf{Pose error prediction accuracy using MAE.} We define $e_{\max}=\max(e_R,e_t)$.}
    \label{tab:verifier_mae}
    \vspace{10pt}

    \small
    \setlength{\tabcolsep}{6pt}
    \renewcommand{\arraystretch}{1.15}

    \begin{tabular}{llccc}
        \toprule
        \textbf{Dataset} 
        & \textbf{Verifier} 
        & \textbf{MAE ($e_R$)} $\downarrow$
        & \textbf{MAE ($e_t$)} $\downarrow$
        & \textbf{MAE($e_{\max}$)} $\downarrow$ \\
        \midrule

        % \multirow{2}{*}{ARKitScenes}
        % & FSNet 
        % & 8.705	& 12.225 & 15.605 \\
        
        % & \rowcolor{gray!10}\textbf{PoseAgent}
        % & \textbf{0.992} & \textbf{5.201} & \textbf{4.520}\\
        
        % \midrule 



        \multirow{2}{*}{MegaDepth}
        & FSNet 
        & 5.463 & 6.615	& 8.588 \\
        
        & \rowcolor{gray!10}\textbf{PoseAgent}
        & \textbf{0.787} & \textbf{4.681} & \textbf{4.243}\\

        \midrule

        \multirow{2}{*}{ScanNet++}
        & FSNet 
        & 34.147
        & 22.934	
        & 41.854 \\

        & \rowcolor{gray!10}\textbf{PoseAgent}
        & \textbf{0.715}	& \textbf{4.316}	& \textbf{2.853} \\

        % \midrule 

        % \multirow{2}{*}{RealEstate10K}
        % & FSNet 
        % & 3.678	& 11.855 & 12.335\\

        % & \rowcolor{gray!10}\textbf{PoseAgent}
        % & \textbf{0.980} & \textbf{2.923} & \textbf{2.780}\\
        

        \bottomrule
    \end{tabular}
\end{table}

==> tables/eval_verifier_ranker+verifier.tex <==
\begin{table*}[t]
    \centering
    % \caption{\textbf{Comparison of ranker Top-1 and verifier-based selection over all candidate models.} }
    \caption{\textbf{Comparison of model selection strategies.} Verifier-only exhausts all models to choose the best predicted hypothesis; Ranker-only only shows Rank-1 model's result. Fixed-order + PVN uses a fixed estimator order for all datasets determined by the dataset average win rate on the training sets, with the same PVN, fallback policy, and $K=4$ as PoseAgent.}
    \label{tab:comp_verifier_only}
    % \vspace{\baselineskip}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lcccccccccccc}
        \toprule

        & \multicolumn{3}{c}{\textbf{ARKitScenes}}
        & \multicolumn{3}{c}{\textbf{MegaDepth}}
        & \multicolumn{3}{c}{\textbf{ScanNet++}}
        & \multicolumn{3}{c}{\textbf{RealEstate10K}} \\

        \cmidrule(lr){2-4}
        \cmidrule(lr){5-7}
        \cmidrule(lr){8-10}
        \cmidrule(lr){11-13}

        \textbf{Model Selection Strategy}
        & \textbf{@5\degree} & \textbf{@10\degree} & \textbf{@20\degree}
        & \textbf{@5\degree} & \textbf{@10\degree} & \textbf{@20\degree}
        & \textbf{@5\degree} & \textbf{@10\degree} & \textbf{@20\degree}
        & \textbf{@5\degree} & \textbf{@10\degree} & \textbf{@20\degree} \\
        \midrule

        
        Verifier-Only
        & 0.455 & 0.669 & 0.813
        & 0.668 & 0.794 & {0.879}
        & {\bf 0.728}	& {\bf 0.856}	& {\bf 0.927}
        & 0.698	& 0.820	& 0.894 \\

        Ranker-Only 
        & {0.460}	& {0.674}	& {0.816}
        & {0.682}	& 0.794	& 0.869	
        & 0.702	& 0.839	& 0.916	
        & {0.729}	& {0.836}	& {0.901} \\

        Fixed-order + PVN
        & 0.467	& 0.681	& 0.821
        & 0.611	& 0.762	& 0.863
        & 0.694	& 0.838	& 0.917
        & 0.636	& 0.786	& 0.875 \\ 

        % \rowcolor{gray!10}
        \rowcolor{red!10}
        PoseAgent (Ranker +  Verifier)
        & \textbf{0.473} & \textbf{0.685} & \textbf{0.823}
        & \textbf{0.693} & \textbf{0.810} & \textbf{0.889}
        & 0.726	& 0.855	& 0.926	
        & \textbf{0.736}	& \textbf{0.843}	& \textbf{0.907} \\

        \midrule
        \rowcolor{gray!7}
        \textit{Oracle@9}
        & 0.607	& 0.778	& 0.881	
        & 0.803	& 0.888	& 0.940	
        & 0.800	& 0.897	& 0.948	
        & 0.829	& 0.900	& 0.941 \\

        
        

        \bottomrule
    \end{tabular}
    }
\end{table*}


==> tables/latency.tex <==
\setlength{\intextsep}{0.5\baselineskip}
\begin{table}[H]
    \centering
    \caption{Average latency per image pair (ms). Model initialization is excluded.}
    % \vspace{\baselineskip}
    \label{tab:module_latency}
    \scriptsize
    \begin{tabular}{lrrrr}
        \toprule
        \textbf{Dataset} & \textbf{Profiling} & \textbf{Ranking} & \textbf{Verifier} \\
        \midrule
        ARKitScenes   & 583.18 & 25.11 & 82.14 \\
        ScanNet++     & 661.42 & 25.70 & 92.09 \\
        MegaDepth     & 691.00 & 25.99 & 90.63 \\
        RealEstate10K & 613.15 & 25.28 & 84.47 \\
        % \midrule
        % Overall (pair-weighted) & -- & -- & -- & -- \\
        \bottomrule
    \end{tabular}
\end{table}

==> tables/vlm_agent_ranker.tex <==
\begin{table}[t]
    \centering
    \captionsetup{font=footnotesize,skip=2pt}
    
    \makebox[\linewidth][c]{%
        % Left table
        \begin{minipage}[c]{0.31\linewidth}
            \vspace{0pt}
            \centering
            \caption{Relative pose estimation on ARKitScenes. Results are AUC@5\degree/10\degree/20\degree.}
            \label{tab:comp_vlm_agent}
            
            \scriptsize
            \setlength{\tabcolsep}{2pt}
            \renewcommand{\arraystretch}{0.95}
            
            \begin{tabular}{@{\hspace{5pt}}lccc@{\hspace{5pt}}}
            \toprule
            % & \multicolumn{3}{c}{\textbf{AUC}} \\
            % \cmidrule(lr){2-4}
            \textbf{Method} & @5 & @10 & @20 \\
            \midrule
            VLM Agent & 0.090 & 0.163 & 0.259 \\
            PoseAgent & \textbf{0.473} & \textbf{0.685} & \textbf{0.823} \\
            \midrule
            Oracle@9 & 0.607 & 0.778 & 0.881 \\
            \bottomrule
            \end{tabular}
        \end{minipage}%
        \hspace{0.02\linewidth}%
        
        % Right table
        \begin{minipage}[c]{0.6\linewidth}
            \vspace{0pt}
            \centering
            \caption{Ranking and verification on ARKitScenes. Both use the same learned verifier and fallback policy with up to four candidates. Results are AUC@5\degree/10\degree/20\degree.}
            \label{tab:vlm_as_ranker}
            
            \scriptsize
            \setlength{\tabcolsep}{2pt}
            \renewcommand{\arraystretch}{0.95}
            
            \begin{tabular}{@{\hspace{10pt}}llccc@{\hspace{10pt}}}
            \toprule
            % & & \multicolumn{3}{c}{\textbf{AUC}} \\
            % \cmidrule(lr){3-5}
            \textbf{Setting} & \textbf{Method} & @5 & @10 & @20 \\
            \midrule
            Rank-1
            & VLM Ranker & 0.369 & 0.549 & 0.691 \\
            & Ranker (Ours) & \textbf{0.460} & \textbf{0.674} & \textbf{0.816} \\
            \midrule
            Oracle@2
            & VLM Ranker & 0.448 & 0.629 & 0.759 \\
            & Ranker (Ours) & \textbf{0.532} & \textbf{0.727} & \textbf{0.851} \\
            \midrule
            PVN + Fallback
            & VLM Ranker & 0.449 & 0.650 & 0.795 \\
            & PoseAgent & \textbf{0.473} & \textbf{0.685} & \textbf{0.823} \\
            \midrule
            Oracle@4
            & VLM & 0.531 & 0.713 & 0.835 \\
            Oracle@9
            & -- & 0.607 & 0.778 & 0.881 \\
            \bottomrule
            \end{tabular}
        \end{minipage}%
    }

\end{table}

==> tables/vlm_as_ranker.tex <==
% \begin{table}[t]
%     \centering
%     \caption{\textbf{Comparison between our ranker and VLM as a ranker on ARKitScenes.} We use Claude-Sonnet-5. }
%     \label{tab:vlm_as_ranker}
%     \vspace{\baselineskip}

%     \begin{tabular}{lccc}
%         \toprule

%         & \multicolumn{3}{c}{\textbf{ARKitScenes}} \\
%         \cmidrule(lr){2-4}

%         \textbf{Ranker}
%         & \textbf{@5}
%         & \textbf{@10}
%         & \textbf{@20} \\
%         \midrule

%         VLM Ranker (Top1) 
%         & 0.369 & 0.549 & 0.691 \\

%         Our Ranker (Top-1)
%         & \textcolor{numred}{\bf 0.460} & \textcolor{numred}{\bf 0.674} & \textcolor{numred}{\bf0.816} \\ 

%         \midrule
%         VLM  (Oracle@2)
%         & 0.448	& 0.629	& 0.759 \\

%         Our Ranker (Oracle@2)
%         & \textcolor{numred}{\bf 0.532} & \textcolor{numred}{\bf 0.727} & \textcolor{numred}{\bf 0.851} \\ 

%         \midrule
%         VLM Ranker + Verifier (Top-4)
%         & 0.449 & 0.650 & 0.795 \\

%         A-CAPE (Top-4)
%         & \textcolor{numred}{\bf 0.473} & \textcolor{numred}{\bf 0.685} & \textcolor{numred}{\bf 0.823} \\

%         \rowcolor{verifierbg}
%         VLM-Calude (Oracle@4)
%         & 0.531 & 0.713 & 0.835 \\

%         \midrule
%         \rowcolor{lightgray}
%         Oracle@9
%         & 0.607 & 0.778 & 0.881 \\ 

%         \bottomrule
%     \end{tabular}
% \end{table}


% \begin{table}[t]
%     \centering
%     \caption{\textbf{Ranking and verification on ARKitScenes} (AUC@5\degree/10\degree/20\degree). Both use the same learned verifier and fallback policy with $K=4$.}
%     \label{tab:vlm_as_ranker}
%     \scriptsize 
%     % \setlength{\tabcolsep}{5pt}
%     \begin{tabular}{llc}
%         \toprule
%         % \multirow{2}{*}{\textbf{Setting}}
%         % & \multirow{2}{*}{\textbf{Method}}
%         % & \multicolumn{3}{c}{\textbf{AUC}} \\
%         % \cmidrule(lr){3-5}
%         % & & @5 & @10 & @20 \\

%         % \textbf{Setting}
%         % & \textbf{Method}
%         % & \textbf{@5\degree}
%         % & \textbf{@10\degree}
%         % & \textbf{@20\degree} \\
        
%          \textbf{Setting}
%         & \textbf{Method}
%         & \textbf{@5\degree/10\degree/20\degree} \\

%         \midrule
        
%         \multirow{2}{*}{Rank-1}
%         & VLM Ranker    
%         & 0.369 / 0.549 / 0.691 \\
        
%         & Ranker (Ours) 
%         & \textbf{0.460 / 0.674 / 0.816} \\
        
%         \midrule
%         \multirow{2}{*}{Oracle@2}
%         & VLM Ranker    
%         & 0.448 / 0.629 / 0.759 \\
%         & Ranker (Ours) 
%         & \textbf{0.532 / 0.727 / 0.851} \\
                  
%         \midrule
%         \multirow{2}{*}{PVN + Fallback}
%         & VLM Ranker     
%         & 0.449 / 0.650 / 0.795 \\
%         & PoseAgent
%         & \textbf{0.473 / 0.685 / 0.823} \\
        
%         % \midrule
%         % \rowcolor{gray!10}
%         % Oracle@4 & VLM & 0.531 & 0.713 & 0.835 \\
%         % \rowcolor{gray!10}
%         % Oracle@9 & --- & 0.607 & 0.778 & 0.881 \\
%         \bottomrule
%     \end{tabular}
% \end{table}

% =========== wraptable ===========
\setlength{\columnsep}{12pt}
\setlength{\intextsep}{5pt}

\begin{wraptable}{r}{0.58\textwidth}
    % \vspace{-8pt}
    \centering
    \captionsetup{font=footnotesize,skip=2pt}
    
    \caption{Ranking and verification on ARKitScenes. Both use the same learned verifier and fallback policy with up to four candidates. Results are AUC@5\degree/10\degree/20\degree.}
    \label{tab:vlm_as_ranker}
    
    \footnotesize
    \setlength{\tabcolsep}{2.5pt}
    \renewcommand{\arraystretch}{0.95}
    
    \begin{tabular}{llccc}
        \toprule

        \textbf{Setting}
        & \textbf{Method}
        & \textbf{@5\degree}
        & \textbf{@10\degree}
        & \textbf{@20\degree} \\

        \midrule
        
        \multirow{2}{*}{Top-1}
        & VLM     & 0.369 & 0.549 & 0.691 \\
        & Ranker (Ours) & \textbf{0.460} & \textbf{0.674}
                  & \textbf{0.816} \\
        \midrule
        \multirow{2}{*}{Oracle@2}
        & VLM     & 0.448 & 0.629 & 0.759 \\
        & Ranker (Ours) & \textbf{0.532} & \textbf{0.727}
                  & \textbf{0.851} \\
        \midrule
        \multirow{2}{*}{Top-4}
        & VLM Ranker + PVN     & 0.449 & 0.650 & 0.795 \\
        & PoseAgent
                  & \textbf{0.473} & \textbf{0.685}
                  & \textbf{0.823} \\
        
        % \midrule
        % \rowcolor{gray!10}
        % Oracle@4 & VLM & 0.531 & 0.713 & 0.835 \\
        % \rowcolor{gray!10}
        % Oracle@9 & --- & 0.607 & 0.778 & 0.881 \\
        \bottomrule
    \end{tabular}
\end{wraptable}
